ARIES: Autonomous Reasoning with LLMs on Interactive Thought Graph Environments

Recent research has shown that LLM performance on reasoning tasks can be enhanced by scaling test-time compute. One promising approach, particularly with decomposable problems, involves arranging intermediate solutions as a graph on which transformations are performed to explore the solution space. However, prior works rely on pre-determined, task-specific transformation schedules which are subject to a set of searched hyperparameters. In this work, we view thought graph transformations as actions in a Markov decision process, and implement policy agents to drive effective action policies for the underlying reasoning LLM agent. In particular, we investigate the ability for another LLM to act as a policy agent on thought graph environments and introduce ARIES, a multi-agent architecture for reasoning with LLMs. In ARIES, reasoning LLM agents solve decomposed subproblems, while policy LLM agents maintain visibility of the thought graph states, and dynamically adapt the problem-solving strategy. Through extensive experiments, we observe that using off-the-shelf LLMs as policy agents with no supervised fine-tuning (SFT) can yield up to $29\%$ higher accuracy on HumanEval relative to static transformation schedules, as well as reducing inference costs by $35\%$ and avoid any search requirements. We also conduct a thorough analysis of observed failure modes, highlighting that limitations on LLM sizes and the depth of problem decomposition can be seen as challenges to scaling LLM-guided reasoning.

==> imgs/main_results.tex <==
\begin{figure}[!th]
\centering
\begin{subfigure}[b]{0.48\textwidth}
\centering
\input{imgs/main_results_matmul}
\caption{Absolute perplexity on SlimPajama at varying quantization ratios.}
\label{fig:main_results_matmul}
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.48\textwidth}
\centering
\input{imgs/main_results_matmul_diff}
\caption{Percentage change in perplexity at varying quantization ratios, relative to non-quantized baseline.}
\label{fig:main_results_matmul_diff}
\end{subfigure}
\caption{Results supporting \textit{LLM-MPQ} Scaling Law 1 at matmul granularity. We show how perplexity on SlimPajama scales with increasing model sizes under various quantization ratios ($Q_r$ values). Larger models can tolerate higher quantization ratios.}
\label{fig:main_results_matmul_overview}
\end{figure}


\begin{figure}[!th]
\centering
\begin{subfigure}[b]{0.48\textwidth}
\centering
\input{imgs/main_results_layerwise}
\caption{Absolute perplexity on SlimPajama at varying quantization ratios.}
\label{fig:main_results_layerwise}
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.48\textwidth}
\centering
\input{imgs/main_results_layerwise_diff}
\caption{Percentage change in perplexity at varying quantization ratios, relative to non-quantized baseline.}
\label{fig:main_results_layerwise_diff}
\end{subfigure}
\caption{Results supporting \textit{LLM-MPQ} Scaling Law 1 at layer granularity. We show how perplexity on SlimPajama scales with increasing model sizes under various quantization ratios ($Q_r$ values). Larger models can tolerate higher quantization ratios.}
\label{fig:main_results_layerwise_overview}
\end{figure}

\begin{figure}[!th]
\centering
\begin{subfigure}[b]{0.48\textwidth}
\centering
\input{imgs/main_results_mmlu_matmul}
\caption{Accuracy on MMLU at varying quantization ratios.}
\label{fig:main_results_mmlu_matmul}
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.48\textwidth}
\centering
\input{imgs/main_results_mmlu_matmul_diff}
\caption{Percentage change in accuracy at varying quantization ratios, relative to non-quantized baseline.}
\label{fig:main_results_mmlu_matmul_diff}
\end{subfigure}
\caption{Results supporting \textit{LLM-MPQ} Scaling Law 1 at matmul granularity. We show how accuracy on MMLU scale with increasing model sizes under various quantization ratios ($Q_r$ values). Bigger models can tolerate higher quantization ratios.}
\label{fig:main_results_mmlu_matmul_overview}
\end{figure}


\begin{figure}[!th]
\centering
\begin{subfigure}[b]{0.48\textwidth}
\centering
\input{imgs/main_results_mmlu_layerwise}
\caption{Accuracy on MMLU at varying quantization ratios.}
\label{fig:main_results_mmlu_layerwise}
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.48\textwidth}
\centering
\input{imgs/main_results_mmlu_layerwise_diff}
\caption{Percentage change in accuracy at varying quantization ratios, relative to non-quantized baseline.}
\label{fig:main_results_mmlu_layerwise_diff}
\end{subfigure}
\caption{Results supporting \textit{LLM-MPQ} Scaling Law 1 at layer granularity. We show how accuracy on MMLU scale with increasing model sizes under various quantization ratios ($Q_r$ values). Bigger models can tolerate higher quantization ratios.}
\vspace{-2em}
\label{fig:main_results_mmlu_layerwise_overview}
\end{figure}



==> imgs/main_results_matmul_diff.tex <==
\begin{tikzpicture}[thick,scale=0.95, every node/.style={scale=0.95}]
\pgfplotsset{every x tick label/.append style={font=\footnotesize}, compat=1.3}
\begin{axis}[
    height=60mm,
    width=\textwidth,
    xlabel={\footnotesize Parameter count (billions)},
    ylabel={\footnotesize $\Delta$Perplexity in \% compared to $Q_r$ = 0},
    ymode=log, 
    log ticks with fixed point, 
    % xmode=log,
    ytick = {1, 0.5, 0.2, 0.1, 0.05},
    yticklabels = {100, 50, 20, 10, 5},
    legend cell align={left},
    legend columns = 2,
    legend style={at={(0.2, 1)},anchor=north west, draw=none, fill=none, font=\footnotesize},
    ]

\addlegendimage{jcred,line width=1pt}
\addlegendentry{qwen}
\addlegendimage{jcblue,line width=1pt}
\addlegendentry{llama2}
\addlegendimage{jcgreen,line width=1pt}
\addlegendentry{gemma2}

\addlegendimage{dashed,line width=1pt,mark=*, mark options={scale=0.5}}
\addlegendentry{$Q_r$ = 0.95}
\addlegendimage{line width=1pt,mark=*, mark options={scale=0.5}}
\addlegendentry{$Q_r$ = 0.99}

\addplot[dashed, jcred, draw=jcred, line width=1pt, mark=*, mark options={scale=0.5}] table
[x=model_size, y=q0.95, col sep=space] {qwen_matmul_pajama_diff.dat};

\addplot[jcred, draw=jcred, line width=1pt, mark=*, mark options={scale=0.5}] table
[x=model_size, y=q0.99, col sep=space] {qwen_matmul_pajama_diff.dat};

\addplot[dashed, jcblue, draw=jcblue, line width=1pt, mark=*, mark options={scale=0.5}] table
[x=model_size, y=q0.95, col sep=space] {llama2_matmul_pajama_diff.dat};

\addplot[jcblue, draw=jcblue, line width=1pt, mark=*, mark options={scale=0.5}] table
[x=model_size, y=q0.99, col sep=space] {llama2_matmul_pajama_diff.dat};

\addplot[dashed, jcgreen, draw=jcgreen, line width=1pt, mark=*, mark options={scale=0.5}] table
[x=model_size, y=q0.95, col sep=space] {gemma2_matmul_pajama_diff.dat};

\addplot[jcgreen, draw=jcgreen, line width=1pt, mark=*, mark options={scale=0.5}] table
[x=model_size, y=q0.99, col sep=space] {gemma2_matmul_pajama_diff.dat};

\end{axis}
\end{tikzpicture}

==> results/gpt4-barchart.tex <==
\begin{figure*}[t]
    \begin{tikzpicture}
 
    \begin{axis} [
        ybar = .05cm,
        bar width = 8pt,
        width=\textwidth,
        height=5.5cm,
        legend style={at={(0,1.15)},anchor=west, draw=none, fill=none, cells={align=left}, yshift=-0.2cm},
        legend columns = 5,
        legend cell align={left},
        xtick = data,
        symbolic x coords={game24, crosswords, sorting, keyword-counting, set-intersection, sudoku},
        xticklabels = {\textbf{game24}, \textbf{crosswords}, \textbf{sorting}, \textbf{keyword-counting}, \textbf{set-intersection}, \textbf{sudoku}},
        ylabel={Accuracy [\%]},
        ylabel style={yshift=-0.3cm},
        nodes near coords, % Adds values on top of bars
        every node near coord/.append style={font=\small, yshift=2pt} % Adjust font size and position
    ]
     
    \addplot table [x=task, y=io] {results/gpt4.dat};
    \addplot table [x=task, y=cot] {results/gpt4.dat};
    \addplot table [x=task, y=tot] {results/gpt4.dat};
    \addplot table [x=task, y=got] {results/gpt4.dat};
    \addplot table [x=task, y=agot] {results/gpt4.dat};
     
    \legend {IO, CoT, ToT, GoT, A-GoT};
     
    \end{axis}
     
    \end{tikzpicture}

    \caption{Task accuracy across various tasks and prompting strategies}
\end{figure*}

==> results/llama-barchart.tex <==
\begin{figure*}[t]
    \label{fig:llama-barchart}
    \begin{tikzpicture}
 
    \begin{axis} [
        ybar = .05cm,
        bar width = 8pt,
        width=\textwidth,
        height=5.5cm,
        legend style={at={(0,1.15)},anchor=west, draw=none, fill=none, cells={align=left}, yshift=-0.2cm},
        legend columns = 5,
        legend cell align={left},
        xtick = data,
        symbolic x coords={sorting32, sorting64, sorting128, set-intersection32, set-intersection64, set-intersection128, keyword-counting},
        xticklabels = {\textbf{sorting32}, \textbf{sorting64}, \textbf{sorting128}, \textbf{set-int32}, \textbf{set-int64}, \textbf{set-int128}, \textbf{keyword-counting}},
        ylabel={Accuracy [\%]},
        ylabel style={yshift=-0.3cm},
        nodes near coords, % Adds values on top of bars
        every node near coord/.append style={font=\small, yshift=2pt},
        ymin=0,
        ymax=120,
    ]
     
    \addplot table [x=task, y=tot] {results/llama-405b.dat};
    \addplot table [x=task, y=got] {results/llama-405b.dat};
    \addplot table [x=task, y=agot] {results/llama-405b.dat};
     
    \legend {ToT, GoT, A-GoT};
     
    \end{axis}
     
    \end{tikzpicture}

    \caption{Task accuracy across various tasks and prompting strategies}
\end{figure*}

==> results/llama-boxplot.tex <==
\begin{tikzpicture}
    \begin{axis}[
    boxplot/draw direction=y,
    ylabel={Score},
    % height=8cm,
    boxplot={
        draw position={1/3 + floor(\plotnumofactualtype/2) + 1/3*mod(\plotnumofactualtype,2)},
        box extend=0.3,
    },
    x=2cm,
    xtick={0,1,2,...,10},
    x tick label as interval,
    xticklabels={
        {sorting32},
        {sorting64},
        {sorting128},
    },
    x tick label style={
        text width=2.5cm,
        align=center
    },
    ]
    
    \pgfplotstableread{results/sorting32_tot.dat}\sortingThirtyTwoTot;
    \pgfplotstableread{results/sorting32_got.dat}\sortingThirtyTwoGot
    \pgfplotstableread{results/sorting32_agot.dat}\sortingThirtyTwoAGot
    
    \pgfplotstableread{results/sorting64_tot.dat}\sortingSixtyFourTot;
    \pgfplotstableread{results/sorting64_got.dat}\sortingSixtyFourGot
    \pgfplotstableread{results/sorting64_agot.dat}\sortingSixtyFourAGot
    
    \pgfplotstableread{results/sorting128_tot.dat}\sortingOneTwentyEightTot;
    \pgfplotstableread{results/sorting128_got.dat}\sortingOneTwentyEightGot
    \pgfplotstableread{results/sorting128_agot.dat}\sortingOneTwentyEightAGot
    
    % Actual boxplots
    \addplot+[
        draw=red,
    ] table[y index=0] {\sortingThirtyTwoGot};
    \addplot+[
        draw=blue,
    ] table[row sep=\\,y index=0] {\sortingThirtyTwoAGot};

    \addplot+[
        draw=red,
    ] table[row sep=\\,y index=0] {\sortingSixtyFourGot};
    \addplot+[
        draw=blue,
    ] table[row sep=\\,y index=0] {\sortingSixtyFourAGot};

    \addplot+[
        draw=red,
    ] table[row sep=\\,y index=0] {\sortingOneTwentyEightGot};
    \addplot+[
        draw=blue,
    ] table[row sep=\\,y index=0] {\sortingOneTwentyEightAGot};

    \end{axis}
\end{tikzpicture}
